Effective field theories for quantum chromo- and electrodynamics

In this dissertation, I introduce the principles and methods of effective field theory and describe my work in three EFTs: First, in the perturbative QCD region, I use soft collinear effective theory (SCET) to prove that strong interaction soft radiation is universal and to increase the QCD accuracy to next-to-next-tonext- to leading logarithm order for new particle searches in hadron colliders. I also compute a new class of non-perturbative, large logarithmic enhancement arising near the elastic limits of deep inelastic scattering and Drell-Yan processes. Second, in the QCD confinement region, I use heavy hadron chiral perturbation theory to study near-threshold enhancements in the scattering of $D$ and $\pi$ mesons near the threshold for the excited $D$-meson state, $D^*$, as well as in the scattering of $D$ and $D^*$ mesons near the threshold for the exotic hadron X(3872). This work provides a clear picture of the hadronic molecule X(3872) and more profound understanding of the nuclear force between hadrons. Finally, inspired by SCET, I construct a new electron-laser effective field theory to describe highly-relativistic electrons traveling in strong laser fields, extract the universal distribution of electrons in strong electromagnetic backgrounds and its evolution in energy from the separated momentum scales of emitted photons and classical radiation, and predict the rate of wide angle photon emission. I conclude with limitations of EFT methods and some perspectives on what new work may be achieved with these EFTs.

==> abstract.tex <==
Effective field theories (EFTs) provide frameworks to systematically improve perturbation expansions in quantum field theory.  This improvement is essential in quantum chromodynamics (QCD) predictions, both at low energy in the description of low momentum hadron-hadron scattering and at high energy in the description of electron-positron, proton-proton, proton-electron collisions.  It is also important in quantum electrodynamics (QED), when electrons interact with a high-intensity, long-wavelength classical field.  I introduce the principles and methods of effective field theory and describe my work in three EFTs:  First, in the perturbative QCD region, I use soft collinear effective theory (SCET) to prove that strong interaction soft radiation is universal and to increase the QCD accuracy to next-to-next-to-next-to leading logarithm order for new particle searches in hadron colliders.  I also compute a new class of non-perturbative, large logarithmic enhancement arising near the elastic limits of deep inelastic scattering and Drell-Yan processes.  Second, in the QCD confinement region, I use heavy hadron chiral perturbation theory to study near-threshold enhancements in the scattering of $D$ and $\pi$ mesons near the threshold for the excited $D$-meson state, $D^*$, as well as in the scattering of $D$ and $D^*$ mesons near the threshold for the exotic hadron X(3872). This work provides a clear picture of the hadronic molecule X(3872) and more profound understanding of the nuclear force between hadrons.  Finally, inspired by SCET, I construct a new electron-laser effective field theory to describe highly-relativistic electrons traveling in strong laser fields, extract the universal distribution of electrons in strong electromagnetic backgrounds and its evolution in energy from the separated momentum scales of emitted photons and classical radiation, and predict the rate of wide angle photon emission.  I conclude with limitations of EFT methods and some perspectives on what new work may be achieved with these EFTs.


==> acknowledgements.tex <==

I would like to thank all my advisors, all my collaborators, all my physics class teachers and all my family and friends.


==> dedication.tex <==
\begin{center}
To my mother and grandfather, Fei and Zhenqing.
\end{center}


